The Curse of Concentration in Robust Learning: Evasion and Poisoning Attacks from Concentration of Measure

Many modern machine learning classifiers are shown to be vulnerable to adversarial perturbations of the instances. Despite a massive amount of work focusing on making classifiers robust, the task seems quite challenging. In this work, through a theoretical study, we investigate the adversarial risk and robustness of classifiers and draw a connection to the well-known phenomenon of concentration of measure in metric measure spaces. We show that if the metric probability space of the test instance is concentrated, any classifier with some initial constant error is inherently vulnerable to adversarial perturbations. One class of concentrated metric probability spaces are the so-called Levy families that include many natural distributions. In this special case, our attacks only need to perturb the test instance by at most $O(\sqrt n)$ to make it misclassified, where $n$ is the data dimension. Using our general result about Levy instance spaces, we first recover as special case some of the previously proved results about the existence of adversarial examples. However, many more Levy families are known (e.g., product distribution under the Hamming distance) for which we immediately obtain new attacks that find adversarial examples of distance $O(\sqrt n)$. Finally, we show that concentration of measure for product spaces implies the existence of forms of "poisoning" attacks in which the adversary tampers with the training data with the goal of degrading the classifier. In particular, we show that for any learning algorithm that uses $m$ training examples, there is an adversary who can increase the probability of any "bad property" (e.g., failing on a particular test instance) that initially happens with non-negligible probability to $\approx 1$ by substituting only $\tilde{O}(\sqrt m)$ of the examples with other (still correctly labeled) examples.

==> Biblio.tex <==
\newcommand{\etalchar}[1]{$^{#1}$}
\begin{thebibliography}{DKK{\etalchar{+}}18b}

\bibitem[ABL17]{awasthi2014powerjournal}
Pranjal Awasthi, Maria{-}Florina Balcan, and Philip~M. Long.
\newblock {The Power of Localization for Efficiently Learning Linear Separators
  with Noise}.
\newblock {\em Journal of the {ACM}}, 63(6):50:1--50:27, 2017.

\bibitem[AKM18]{attias2018improved}
Idan Attias, Aryeh Kontorovich, and Yishay Mansour.
\newblock Improved generalization bounds for robust learning.
\newblock {\em arXiv preprint arXiv:1810.02180}, 2018.

\bibitem[AM80]{amir1980unconditional}
D~Amir and VD~Milman.
\newblock Unconditional and symmetric sets inn-dimensional normed spaces.
\newblock {\em Israel Journal of Mathematics}, 37(1-2):3--20, 1980.

\bibitem[AM85]{alon1985lambda1}
Noga Alon and Vitali~D Milman.
\newblock $\lambda$1, isoperimetric inequalities for graphs, and
  superconcentrators.
\newblock {\em Journal of Combinatorial Theory, Series B}, 38(1):73--88, 1985.

\bibitem[BCM{\etalchar{+}}13]{Evasion:TestTime}
Battista Biggio, Igino Corona, Davide Maiorca, Blaine Nelson, Nedim Srndic,
  Pavel Laskov, Giorgio Giacinto, and Fabio Roli.
\newblock {Evasion Attacks against Machine Learning at Test Time}.
\newblock In {\em ECML/PKDD}, pages 387--402, 2013.

\bibitem[BE02]{bousquet2002stability}
Olivier Bousquet and Andr{\'e} Elisseeff.
\newblock Stability and generalization.
\newblock {\em Journal of machine learning research}, 2(Mar):499--526, 2002.

\bibitem[BEK02]{NastyNoise}
Nader~H. Bshouty, Nadav Eiron, and Eyal Kushilevitz.
\newblock {{PAC} learning with nasty noise}.
\newblock {\em Theoretical Computer Science}, 288(2):255--275, 2002.

\bibitem[BFR14]{biggio2014security}
Battista Biggio, Giorgio Fumera, and Fabio Roli.
\newblock Security evaluation of pattern classifiers under attack.
\newblock {\em IEEE transactions on knowledge and data engineering},
  26(4):984--996, 2014.

\bibitem[BNL12]{biggio2012poisoning}
Battista Biggio, Blaine Nelson, and Pavel Laskov.
\newblock Poisoning attacks against support vector machines.
\newblock In {\em Proceedings of the 29th International Coference on
  International Conference on Machine Learning}, pages 1467--1474. Omnipress,
  2012.

\bibitem[BNS{\etalchar{+}}06]{barreno2006can}
Marco Barreno, Blaine Nelson, Russell Sears, Anthony~D Joseph, and J~Doug
  Tygar.
\newblock Can machine learning be secure?
\newblock In {\em Proceedings of the 2006 ACM Symposium on Information,
  computer and communications security}, pages 16--25. ACM, 2006.

\bibitem[Bor75]{borell1975brunn}
Christer Borell.
\newblock The brunn-minkowski inequality in gauss space.
\newblock {\em Inventiones mathematicae}, 30(2):207--216, 1975.

\bibitem[BPR18]{bubeck2018adversarial}
S{\'e}bastien Bubeck, Eric Price, and Ilya Razenshteyn.
\newblock {Adversarial examples from computational constraints}.
\newblock {\em arXiv preprint arXiv:1805.10204}, 2018.

\bibitem[CSV17]{charikar2017learning}
Moses Charikar, Jacob Steinhardt, and Gregory Valiant.
\newblock Learning from untrusted data.
\newblock In {\em Proceedings of the 49th Annual ACM SIGACT Symposium on Theory
  of Computing}, pages 47--60. ACM, 2017.

\bibitem[CW17]{CarliniWagner}
Nicholas Carlini and David~A. Wagner.
\newblock {Towards Evaluating the Robustness of Neural Networks}.
\newblock In {\em 2017 {IEEE} Symposium on Security and Privacy, {SP} 2017, San
  Jose, CA, USA, May 22-26, 2017}, pages 39--57, 2017.

\bibitem[DKK{\etalchar{+}}16]{diakonikolas2016robust}
Ilias Diakonikolas, Gautam Kamath, Daniel~M Kane, Jerry Li, Ankur Moitra, and
  Alistair Stewart.
\newblock Robust estimators in high dimensions without the computational
  intractability.
\newblock In {\em Foundations of Computer Science (FOCS), 2016 IEEE 57th Annual
  Symposium on}, pages 655--664. IEEE, 2016.

\bibitem[DKK{\etalchar{+}}17]{diakonikolas2017being}
Ilias Diakonikolas, Gautam Kamath, Daniel~M Kane, Jerry Li, Ankur Moitra, and
  Alistair Stewart.
\newblock Being robust (in high dimensions) can be practical.
\newblock In {\em International Conference on Machine Learning}, pages
  999--1008, 2017.

\bibitem[DKK{\etalchar{+}}18a]{diakonikolas2018robustly}
Ilias Diakonikolas, Gautam Kamath, Daniel~M Kane, Jerry Li, Ankur Moitra, and
  Alistair Stewart.
\newblock Robustly learning a gaussian: Getting optimal error, efficiently.
\newblock In {\em Proceedings of the Twenty-Ninth Annual ACM-SIAM Symposium on
  Discrete Algorithms}, pages 2683--2702. Society for Industrial and Applied
  Mathematics, 2018.

\bibitem[DKK{\etalchar{+}}18b]{diakonikolas2018sever}
Ilias Diakonikolas, Gautam Kamath, Daniel~M Kane, Jerry Li, Jacob Steinhardt,
  and Alistair Stewart.
\newblock Sever: A robust meta-algorithm for stochastic optimization.
\newblock {\em arXiv preprint arXiv:1803.02815}, 2018.

\bibitem[DKS17]{diakonikolas2017statistical}
Ilias Diakonikolas, Daniel~M Kane, and Alistair Stewart.
\newblock Statistical query lower bounds for robust estimation of
  high-dimensional {G}aussians and {G}aussian mixtures.
\newblock In {\em Foundations of Computer Science (FOCS), 2017 IEEE 58th Annual
  Symposium on}, pages 73--84. IEEE, 2017.

\bibitem[DKS18a]{diakonikolas2018list}
Ilias Diakonikolas, Daniel~M Kane, and Alistair Stewart.
\newblock List-decodable robust mean estimation and learning mixtures of
  spherical {G}aussians.
\newblock In {\em Proceedings of the 50th Annual ACM SIGACT Symposium on Theory
  of Computing}, pages 1047--1060. ACM, 2018.

\bibitem[DKS18b]{diakonikolas2018efficient}
Ilias Diakonikolas, Weihao Kong, and Alistair Stewart.
\newblock Efficient algorithms and lower bounds for robust linear regression.
\newblock {\em arXiv preprint arXiv:1806.00040}, 2018.

\bibitem[DMM18]{Adversarial:NIPS}
Dimitrios~I. Diochnos, Saeed Mahloujifar, and Mohammad Mahmoody.
\newblock {Adversarial Risk and Robustness: General Definitions and
  Implications for the Uniform Distribution}.
\newblock In {\em Conference on Neural Information Processing Systems (NIPS)},
  2018.

\bibitem[FFF18]{fawzi2018adversarial}
Alhussein Fawzi, Hamza Fawzi, and Omar Fawzi.
\newblock {Adversarial vulnerability for any classifier}.
\newblock {\em arXiv preprint arXiv:1802.08686}, 2018.

\bibitem[FMS15]{feige2015learning}
Uriel Feige, Yishay Mansour, and Robert Schapire.
\newblock Learning and inference in the presence of corrupted inputs.
\newblock In {\em Conference on Learning Theory}, pages 637--657, 2015.

\bibitem[FMS18]{feige2018robust}
Uriel Feige, Yishay Mansour, and Robert~E Schapire.
\newblock Robust inference for multiclass classification.
\newblock In {\em Algorithmic Learning Theory}, pages 368--386, 2018.

\bibitem[GM01]{giannopoulos2001euclidean}
Apostolos~A Giannopoulos and Vitali~D Milman.
\newblock {Euclidean structure in finite dimensional normed spaces}.
\newblock {\em Handbook of the geometry of Banach spaces}, 1:707--779, 2001.

\bibitem[GMF{\etalchar{+}}18]{gilmer2018adversarial}
Justin Gilmer, Luke Metz, Fartash Faghri, Samuel~S Schoenholz, Maithra Raghu,
  Martin Wattenberg, and Ian Goodfellow.
\newblock {Adversarial Spheres}.
\newblock {\em arXiv preprint arXiv:1801.02774}, 2018.

\bibitem[GMP18]{GoodfellowEtAl:MakeMLRobust}
Ian~J. Goodfellow, Patrick~D. McDaniel, and Nicolas Papernot.
\newblock {Making machine learning robust against adversarial inputs}.
\newblock {\em Communications of the {ACM}}, 61(7):56--66, 2018.

\bibitem[GSS15]{Adversarial::Harnessing}
Ian Goodfellow, Jonathon Shlens, and Christian Szegedy.
\newblock {Explaining and Harnessing Adversarial Examples}.
\newblock In {\em ICLR}, 2015.

\bibitem[Har66]{harper1966optimal}
Lawrence~H Harper.
\newblock Optimal numberings and isoperimetric problems on graphs.
\newblock {\em Journal of Combinatorial Theory}, 1(3):385--393, 1966.

\bibitem[KL93]{KearnsLi::Malicious}
Michael~J. Kearns and Ming Li.
\newblock {Learning in the Presence of Malicious Errors}.
\newblock {\em {SIAM} Journal on Computing}, 22(4):807--837, 1993.

\bibitem[KL17]{koh2017understanding}
Pang~Wei Koh and Percy Liang.
\newblock Understanding black-box predictions via influence functions.
\newblock In {\em International Conference on Machine Learning}, pages
  1885--1894, 2017.

\bibitem[Led01]{ledoux2001concentration}
Michel Ledoux.
\newblock {\em {The Concentration of Measure Phenomenon}}.
\newblock Number~89 in Mathematical Surveys and Monographs. American
  Mathematical Society, 2001.

\bibitem[L{\'e}v51]{levy1951problemes}
Paul L{\'e}vy.
\newblock {\em Probl{\`e}mes concrets d'analyse fonctionnelle}, volume~6.
\newblock Gauthier-Villars Paris, 1951.

\bibitem[LRV16]{lai2016agnostic}
Kevin~A Lai, Anup~B Rao, and Santosh Vempala.
\newblock Agnostic estimation of mean and covariance.
\newblock In {\em Foundations of Computer Science (FOCS), 2016 IEEE 57th Annual
  Symposium on}, pages 665--674. IEEE, 2016.

\bibitem[MDM18]{Mahloujifar2018:ALT}
Saeed Mahloujifar, Dimitrios~I Diochnos, and Mohammad Mahmoody.
\newblock {Learning under $p$-Tampering Attacks}.
\newblock In {\em ALT}, pages 572--596, 2018.

\bibitem[MM17]{pTampTCC17}
Saeed Mahloujifar and Mohammad Mahmoody.
\newblock {Blockwise p-Tampering Attacks on Cryptographic Primitives,
  Extractors, and Learners}.
\newblock In {\em Theory of Cryptography Conference}, pages 245--279. Springer,
  2017.

\bibitem[MMS{\etalchar{+}}18]{madry2017towards}
Aleksander Madry, Aleksandar Makelov, Ludwig Schmidt, Dimitris Tsipras, and
  Adrian Vladu.
\newblock {Towards Deep Learning Models Resistant to Adversarial Attacks}.
\newblock In {\em ICLR}, 2018.

\bibitem[MRT15]{mansour2015robust}
Yishay Mansour, Aviad Rubinstein, and Moshe Tennenholtz.
\newblock Robust probabilistic inference.
\newblock In {\em Proceedings of the twenty-sixth annual ACM-SIAM symposium on
  Discrete algorithms}, pages 449--460. Society for Industrial and Applied
  Mathematics, 2015.

\bibitem[MS86]{milman1986asymptotic}
Vitali~D Milman and Gideon Schechtman.
\newblock {\em Asymptotic theory of finite dimensional normed spaces}, volume
  1200.
\newblock Springer Verlag, 1986.

\bibitem[PMSW16]{papernot2016towards}
Nicolas Papernot, Patrick McDaniel, Arunesh Sinha, and Michael Wellman.
\newblock Towards the science of security and privacy in machine learning.
\newblock {\em arXiv preprint arXiv:1611.03814}, 2016.

\bibitem[PMW{\etalchar{+}}16]{Defenses:Distillation}
Nicolas Papernot, Patrick~D. McDaniel, Xi~Wu, Somesh Jha, and Ananthram Swami.
\newblock {Distillation as a Defense to Adversarial Perturbations Against Deep
  Neural Networks}.
\newblock In {\em {IEEE} Symposium on Security and Privacy, {SP} 2016, San
  Jose, CA, USA, May 22-26, 2016}, pages 582--597, 2016.

\bibitem[PSBR18]{prasad2018robust}
Adarsh Prasad, Arun~Sai Suggala, Sivaraman Balakrishnan, and Pradeep Ravikumar.
\newblock Robust estimation via robust gradient estimation.
\newblock {\em arXiv preprint arXiv:1802.06485}, 2018.

\bibitem[RNH{\etalchar{+}}09]{rubinstein2009antidote}
Benjamin~I.P. Rubinstein, Blaine Nelson, Ling Huang, Anthony~D. Joseph,
  Shing-hon Lau, Satish Rao, Nina Taft, and J.D. Tygar.
\newblock Antidote: understanding and defending against poisoning of anomaly
  detectors.
\newblock In {\em Proceedings of the 9th ACM SIGCOMM conference on Internet
  measurement conference}, pages 1--14. ACM, 2009.

\bibitem[SST{\etalchar{+}}18]{schmidt2018adversarially}
Ludwig Schmidt, Shibani Santurkar, Dimitris Tsipras, Kunal Talwar, and
  Aleksander Madry.
\newblock {Adversarially Robust Generalization Requires More Data}.
\newblock {\em arXiv preprint arXiv:1804.11285}, 2018.

\bibitem[ST78]{sudakov1978extremal}
Vladimir~N Sudakov and Boris~S Tsirel'son.
\newblock Extremal properties of half-spaces for spherically invariant
  measures.
\newblock {\em Journal of Soviet Mathematics}, 9(1):9--18, 1978.

\bibitem[STS16]{shen2016uror}
Shiqi Shen, Shruti Tople, and Prateek Saxena.
\newblock A uror: defending against poisoning attacks in collaborative deep
  learning systems.
\newblock In {\em Proceedings of the 32nd Annual Conference on Computer
  Security Applications}, pages 508--519. ACM, 2016.

\bibitem[SZS{\etalchar{+}}14]{Szegedy:intriguing}
Christian Szegedy, Wojciech Zaremba, Ilya Sutskever, Joan Bruna, Dumitru Erhan,
  Ian Goodfellow, and Rob Fergus.
\newblock {Intriguing properties of neural networks}.
\newblock In {\em ICLR}, 2014.

\bibitem[Tal95]{talagrand1995concentration}
Michel Talagrand.
\newblock Concentration of measure and isoperimetric inequalities in product
  spaces.
\newblock {\em Publications Math{\'e}matiques de l'Institut des Hautes Etudes
  Scientifiques}, 81(1):73--205, 1995.

\bibitem[Val85]{Valiant::DisjunctionsConjunctions}
Leslie~G. Valiant.
\newblock {Learning disjunctions of conjunctions}.
\newblock In {\em IJCAI}, pages 560--566, 1985.

\bibitem[WC18]{PoisoningOnlineWangChaudhuri}
Yizhen Wang and Kamalika Chaudhuri.
\newblock {Data Poisoning Attacks against Online Learning}.
\newblock {\em arXiv preprint arXiv:1808.08994}, 2018.

\bibitem[XBB{\etalchar{+}}15]{xiao2015feature}
Huang Xiao, Battista Biggio, Gavin Brown, Giorgio Fumera, Claudia Eckert, and
  Fabio Roli.
\newblock Is feature selection secure against training data poisoning?
\newblock In {\em ICML}, pages 1689--1698, 2015.

\bibitem[XEQ18]{Adversarial::FeatureSqueezing}
Weilin Xu, David Evans, and Yanjun Qi.
\newblock {Feature Squeezing: Detecting Adversarial Examples in Deep Neural
  Networks}.
\newblock In {\em NDSS}, 2018.

\end{thebibliography}

